MoTE: Reconciling Generalization with Specialization for Visual-Language to Video Knowledge Transfer

Transferring visual-language knowledge from large-scale foundation models for video recognition has proved to be effective. To bridge the domain gap, additional parametric modules are added to capture the temporal information. However, zero-shot generalization diminishes with the increase in the number of specialized parameters, making existing works a trade-off between zero-shot and close-set performance. In this paper, we present MoTE, a novel framework that enables generalization and specialization to be balanced in one unified model. Our approach tunes a mixture of temporal experts to learn multiple task views with various degrees of data fitting. To maximally preserve the knowledge of each expert, we propose \emph{Weight Merging Regularization}, which regularizes the merging process of experts in weight space. Additionally with temporal feature modulation to regularize the contribution of temporal feature during test. We achieve a sound balance between zero-shot and close-set video recognition tasks and obtain state-of-the-art or competitive results on various datasets, including Kinetics-400 \& 600, UCF, and HMDB. Code is available at \url{https://github.com/ZMHH-H/MoTE}.

==> 010_introduction.tex <==
\section{Introduction}
\label{Sec::Introduction}

In the field of deep neural networks, \emph{generalization} and \emph{specialization} are widely regarded as key indicators in reflecting the quality of the model.
Over the past decades, conventional supervised learning, optimized with manually labeled data and task-specific objectives, has showcased remarkable specialization capabilities tailored for specific tasks~\cite{ResNet,Transformer,I3D}.
Recently, Vision-Language Models (VLMs) have demonstrated superior generalization capabilities (e.g., CLIP~\cite{CLIP}, ALIGN~\cite{ALIGN}, Florence~\cite{Florence}). 
Their semantic visual concepts empowered by aligning large-scale image-text pairs can be transferred to a variety of downstream tasks, such as classification~\cite{CoOp,Tipadapter}, segmentation~\cite{Groupvit}, and detection~\cite{ViLD}.

Naturally, video recognition task can also benefits from transferring such powerful visual-language knowledge to the video domain.
The starting point of this transfer paradigm is a well-generalized VLM, with the aim of yielding a model specialized in the video domain.
Depending on the requirements of generalization and specialization set by various task settings, explorations in this field can be summarized as seeking a trade-off between the two aspects.
From this perspective, existing methods can be divided into two lines.
% One line focuses on preserving the generalization of the original VLM by keeping its structure intact~\cite{OpenVCLIP,ViFiCLIP} or adding a few trainable prompts~\cite{VitaCLIP,SiF}.
One line focuses on preserving the generalization by applying minimal structural modification to the VLM, such as keeping its structure intact~\cite{OpenVCLIP,ViFiCLIP} or adding a few 
% These methods excel in zero-shot tasks, which require strong generalization to identify unseen video categories.
The other line adds extra temporal modules on top of the VLM for more specialized temporal modeling~\cite{XCLIP,Text4vis,BIKE}.
% However, more specialized parameters typically come at the cost of diminished generalization, since the fine-tuning video dataset is substantially smaller than the pre-training dataset of VLMs.
We provide an overview of existing methods in Figure~\ref{Fig::teaser}.
Interestingly, we observe a clear trade-off trend between zero-shot and close-set performance, but no method achieves the best of both worlds.
This leads us one step further: \emph{Can generalization and specialization coexist well in one model when transferring VLMs to the video domain?}

% ----------------- figure-------------------------
\begin{figure*}[t]
\begin{center}
\centerline{
    \includegraphics[width=\linewidth]{Figures/teaser_all.pdf}}
\caption{Overview of existing VLM knowledge transfer methods. (a) Existing methods constrain the transferred video model to learn a feature space geared towards either zero-shot or close-set tasks. Our proposed MoTE seeks to construct a reconciled feature space between the two optimal solution manifolds. (b) Trade-off plots between zero-shot and close-set performance of recent CLIP-based methods (ViT-B/16). MoTE achieves an optimal balance between the two aspects. Marker shapes represent the ways for temporal modeling.}
% Please zoom in for the best view.}
\label{Fig::teaser}
\end{center}
\vskip -0.2in
\end{figure*}
% --------------------------------------------------

It is worth noting that when transferring VLMs to downstream tasks, extra adaptation modules are commonly applied to bridge the gap between the source and target domains~\cite{ActionClip,ClipCap,PointCLIP}.
However, these newly added parameters tend to overfit the target domain, since (\romannumeral1) they are typically initialized with random weights and (\romannumeral2) the fine-tuning dataset is substantially smaller than the pre-training dataset of VLMs.
% However, the newly added parameters tend to overfit the target domain for two reasons.
% Firstly, these parameters are typically initialized with random weights, which does not provide a generalized starting point for transferring. 
% Secondly, the fine-tuning dataset is substantially smaller than the pre-training dataset of VLMs. 
As a consequence, more specialized parameters typically come at the cost of diminished generalization of the original VLM. 
While previous studies suggest that non-parametric (e.g., temporal pooling) or prompt-based methods are insufficient for modeling the complex temporal dynamics in the video, this motivates us to seek a way that improves the generalization of the extra temporal module without reducing its specialized temporal modeling capability.

In this paper, we present MoTE, a mixture of temporal experts approach with well-balanced generalization and specialization.
% we take inspiration from MoE to induce sparsity
In contrast to traditional temporal modules that encode patterns with a \emph{single} feedforward network (FFN) in each Transformer layer, MoTE uses \emph{multiple} FFNs and treats each of them as a temporal expert.
We induce sparsity by routing incoming frame token sequences to one of the temporal experts. 
This property also keeps the computational cost the same as using a single FFN. We design a multinomial distribution-based routing algorithm that enables experts to learn multiple task views with different degrees of generalization. During inference, we adopt a weights merging strategy~\cite{modelsoups,adamix} to collapse multiple experts into one module.
While each individual expert contributes diverse knowledge, we further propose a \emph{Weight Merging Regularization} that drives a range of the merged parameters optimal with respect to the task-specific objective.
This enables the merged model to retain the generalization of each expert with almost no degradation of temporal modeling capability.
To further alleviate the overfitting at test time, we devise a plug-and-play module that modulates the contribution of temporal features by measuring the semantic association between the proxy text features from the fine-tuning and the test datasets.

We conduct extensive experiments to evaluate the performance of MoTE on zero-shot benchmarks (i.e., UCF-101, HMDB-51, and Kinetics-600) and a close-set benchmark (i.e., Kinetics-400).
MoTE demonstrates a sound balance between zero-shot and close-set performance.
In particular, we achieve state-of-the-art or competitive results on both tasks with one unified model, even compared to methods tailored for a single task.
Further analysis shows the scalability and effectiveness of our proposed approach.
% % 太长了
% Our main contributions can be summarized as follows:
% % \begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
% \begin{itemize}[noitemsep,topsep=0pt]
% \item We propose MoTE, a Mixture-of-Temporal-Experts approach for transferring visual-language knowledge to the video domain.
% \item We present Weight Merging Regularization, a novel regularizer to retain the generalization of underlying MoE architecture while prompting specialized temporal modeling ability. Together with a distribution-based routing algorithm and feature adjustment module to further improve the generalization of MoTE.
% \item We conduct extensive experiments to demonstrate the performance of MoTE. MoTE achieves state-of-the-art or competitive performance on both zero-shot and close-set tasks, even compared to methods tailored for a single task.
% \end{itemize}

==> 011_bak.tex <==
% ------------------------ zero shot bak --------------------------------
\begin{table*}[t]
\renewcommand\arraystretch{0.98}
\caption{Zero-shot classification performance compared with the state-of-the-art methods on UCF-101, HMDB-51, and Kinetics-600. We compare with two protocols on UCF-101 and HMDB51, i.e., full dataset evaluation and splits evaluation.}
\label{Tab::Zeroshot}
% \vskip 0.1in
\begin{center}
\begin{footnotesize}
% \scalebox{1.2}[1.2]{
\resizebox{0.82\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
Method                         & Encoder   & Protocol & UCF-101 & HMDB-51 & Kinetics-600\\
\midrule
E2E~\cite{E2E}                 & R(2+1)D   & Full     & 37.6    &    -    & -           \\
ER~\cite{ER}                   & TSM       & Full     & -       &    -    & 42.1        \\
ResT~\cite{ResT}               & ResNet101 & Full     & 40.6    & 34.4    & -           \\
\midrule
\multicolumn{6}{l}{\textit{Generalization-oriented transfer methods}} \\
OTI~\cite{OTI}                 & ViT-B/32  & Full     & 79.0    & 49.9    & 64.5$\pm$1.1  \\
OTI~\cite{OTI}                 & ViT-B/16  & Full     & 83.7    & 51.0    & 66.9$\pm$1.0  \\
OTI~\cite{OTI}                 & ViT-L/14  & Full     & 88.3    & 55.8    & 70.6$\pm$0.5  \\
Open-VCLIP~\cite{OpenVCLIP}    & ViT-B/32  & Full     & 79.5    & 49.9    & 69.5$\pm$0.6  \\
Open-VCLIP~\cite{OpenVCLIP}    & ViT-B/16  & Full     & 83.5    & 53.2    & 73.0$\pm$0.8  \\
Open-VCLIP~\cite{OpenVCLIP}    & ViT-L/14  & Full     & 87.9    & 58.3    & 81.1$\pm$0.8  \\
\midrule
\multicolumn{6}{l}{\textit{Specialization-oriented transfer methods}} \\
ActionCLIP~\cite{ActionClip}   & ViT-B/16  & Full     & 69.5    & 50.5    & -             \\
Text4Vis~\cite{Text4vis}       & ViT-L/14  & Full     & 79.6    & 49.8    & 68.9$\pm$1.0  \\
BIKE~\cite{BIKE}               & ViT-L/14  & Full     & 80.8    & 52.8    & 68.5$\pm$1.2  \\
\midrule
\multicolumn{6}{l}{\textit{Balance-oriented transfer methods}} \\
\textbf{MoTE (ours)}           & ViT-B/32  & Full     & 80.8    & 49.3  &  66.7$\pm$0.5  \\
\textbf{MoTE (ours)}           & ViT-B/16  & Full     & 83.4    & 51.0  &  69.2$\pm$0.7  \\
\textbf{MoTE (ours)}           & ViT-L/14  & Full     & 89.4    & 56.3  &  78.0$\pm$0.9  \\
\midrule
A5~\cite{A5}                   & ViT-B/16  & Splits   & 69.3$\pm$4.2  & 44.3$\pm$2.2    & -            \\
X-CLIP~\cite{XCLIP}            & ViT-B/16  & Splits   & 72.0$\pm$2.3  & 44.6$\pm$5.2    & 65.2$\pm$0.4 \\
Vita-CLIP~\cite{VitaCLIP}      & ViT-B/16  & Splits   & 75.0$\pm$0.6  & 48.6$\pm$0.6    & 67.4$\pm$0.5 \\
\textbf{MoTE (ours)}           & ViT-B/16  & Splits   & 83.4$\pm$0.3  & 53.7$\pm$0.2    &  69.2$\pm$0.7\\
\bottomrule
\end{tabular}
}
\end{footnotesize}
\end{center}
\vskip -0.1in
\end{table*}



% ------------------ close-set performance------------------
\begin{table*}[t]
\renewcommand\arraystretch{0.98}
\caption{Close-set classification result compared with the state-of-the-art methods on Kinetics-400.}
\label{Tab::Closeset}
% \vskip 0.1in
\begin{center}
\begin{scriptsize}
% \scalebox{1.2}[1.2]{
\resizebox{0.88\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
Method                         & Encoder  & Pre-training & Input Size    & Views      & Top-1 & Top-5 \\
\midrule
TimeSformer~\cite{TimeSformer} & ViT-L    & ImageNet-21K & 96$\times$224 & 1$\times$3 & 80.7  & 94.7  \\
% MViT~\cite{MViT}               & MViT-B   &     -        & 64$\times$224 & 5$\times$1 & 81.2  & 95.1  \\
Video Swin~\cite{ViViT}        & Swin-L   & ImageNet-21K & 32$\times$224 & 4$\times$3 & 83.1  & 95.9  \\
ViViT FE~\cite{ViViT}          & ViT-L    & ImageNet-21K & 128$\times$224& 1$\times$3 & 81.7  & 93.8  \\
\midrule
\multicolumn{7}{l}{\textit{Generalization-oriented transfer methods}} \\
A6~\cite{A5}                   & ViT-B/16 & CLIP-400M    & 16$\times$224 &    -       & 76.9  & 93.5   \\
SiF~\cite{SiF}                 & ViT-B/16 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 77.4  & 93.6   \\
Open-VCLIP~\cite{OpenVCLIP}    & ViT-B/16 & CLIP-400M    & 8$\times$224  & 1$\times$1 & 78.9  &   -    \\
\midrule
\multicolumn{7}{l}{\textit{Specialization-oriented transfer methods}} \\
% X-CLIP~\cite{XCLIP}            & ViT-B/16 & CLIP-400M    & $8\times224$  & $1\times1$ & 82.3  & 95.8   \\
X-CLIP~\cite{XCLIP}            & ViT-B/16 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 83.8  & 96.7   \\
X-CLIP~\cite{XCLIP}            & ViT-L/14 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 87.1  & 97.6   \\
BIKE~\cite{BIKE}               & ViT-L/14 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 87.4  &  -     \\
Text4Vis~\cite{Text4vis}       & ViT-B/16 & CLIP-400M    & 8$\times$224  & 1$\times$1 & 81.5  & 95.5   \\
Text4Vis~\cite{Text4vis}       & ViT-B/16 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 82.9  &  -     \\
Text4Vis~\cite{Text4vis}       & ViT-L/14 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 86.4  &  -     \\
\midrule
\multicolumn{7}{l}{\textit{Balance-oriented transfer methods}} \\
Vita-CLIP~\cite{VitaCLIP}      & ViT-B/16 & CLIP-400M    & 8$\times$224  & 1$\times$1 & 80.5  &  95.9  \\
Vita-CLIP~\cite{VitaCLIP}      & ViT-B/16 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 81.8  &  96.0  \\
\textbf{MoTE (ours)}           & ViT-B/16 & CLIP-400M    & 8$\times$224  & 1$\times$1 & 81.6  &  95.3  \\
\textbf{MoTE (ours)}           & ViT-B/16 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 82.7  &  96.2  \\
\textbf{MoTE (ours)}           & ViT-L/14 & CLIP-400M    & 8$\times$224  & 4$\times$3 & 86.3  &  97.6  \\
\bottomrule
\end{tabular}
}
\end{scriptsize}
\end{center}
\vskip -0.1in
\end{table*}


\begin{table}[ht]
\renewcommand\arraystretch{0.98}
\caption{Comparing the trade-off between close-set performance and zero-shot performance. HM indicates the harmonic mean of UCF-101, HMDB-51, and Kinetics-600.}
\label{Tab::Tradeoff}
\vskip 0.1in
\begin{center}
\begin{Large}
% \begin{sc}
% \scalebox{1.2}[1.2]{
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
Method               & Temporal Modeling   & Encoder   & K400   & HM  \\
\midrule
Open-VCLIP           & Non-parametric    & ViT-B/16  & 78.9   & \textbf{67.5}    \\
Vita-CLIP            & Prompt-based      & ViT-B/16  & 80.5   & 61.5    \\
Text4Vis             & Temporal module   & ViT-B/16  & 81.5   & 56.4    \\
\textbf{MoTE (ours)} & Temporal module   & ViT-B/16  & \textbf{81.6}   & 65.2    \\
\bottomrule
\end{tabular}
}
% \end{sc}
\end{Large}
\end{center}
\vskip -0.1in
\end{table}

==> 10_ckecklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: Our main contributions are detailed in lines 6-14 of the abstract and lines 67-77 of the introduction.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: We analyze the limitations of this paper in Section \ref{Appendix::Sec::Limitation} of the Appendix.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: As an applied paper, we aim to provide a more generalized and effective VLMs knowledge transfer framework for video recognition tasks. We do not include theoretical results in this paper. Note that all assumptions and conclusions mentioned in this paper are precisely cited.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results. 
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    % \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: We detail the implementation details of the paper in Section \ref{Sec::Experiments::Setup} of the main manuscript and Section \ref{Appendix::Sec::details} of the Appendix. Besides, we provide our code in the supplementary zip file. The code will also be released when the paper is accepted.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: We provide our code in the supplementary zip file with a detailed instruction to reproduce our method. The code will also be released when the paper is accepted.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: We specify all training and evaluation details of our method in Section \ref{Sec::Experiments::Setup} of the main manuscript and Section \ref{Appendix::Sec::details} of the Appendix.
    We also provide statistics details for the dataset used in this paper in Section \ref{Appendix::Sec::Dataset} of the Appendix.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}, % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For zero-shot experiments, following the previous works, we evaluate our method on three splits of UCF-101, HMDB-51, and K600. We report the mean accuracy and the standard deviation of performance of the three splits on each dataset, respectively. As for close-set and few-shot experiments, considering the computational effort, we do not include error bars following previous works.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] 
    Justification: 
    We report computational resources and training costs in Section \ref{Appendix::Sec::details} and Section \ref{Appendix::Sec::Ablations} of the Appendix.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: : All authors have read the NeurIPS Code of Ethics.

\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    We discuss the potential broader impacts in Section \ref{Appendix::Sec::Limitation} of the Appendix.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
     This paper poses no such risks.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    All references and datasets in this paper are precisely cited and licensed with corresponding licenses.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    We provide detailed instructions on submitted assets. The details of the dataset and model are reported in our paper.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    This paper does not involve crowdsourcing nor research with human subjects.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    This paper poses no such risks.

\end{enumerate}
